Leveraging Semantic Web Technologies for Managing Resources in a Multi-Domain Infrastructure-as-a-Service Environment

This paper reports on experience with using semantically-enabled network resource models to construct an operational multi-domain networked infrastructure-as-a-service (NIaaS) testbed called ExoGENI, recently funded through NSF's GENI project. A defining property of NIaaS is the deep integration of network provisioning functions alongside the more common storage and computation provisioning functions. Resource provider topologies and user requests can be described using network resource models with common base classes for fundamental cyber-resources (links, nodes, interfaces) specialized via virtualization and adaptations between networking layers to specific technologies. This problem space gives rise to a number of application areas where semantic web technologies become highly useful - common information models and resource class hierarchies simplify resource descriptions from multiple providers, pathfinding and topology embedding algorithms rely on query abstractions as building blocks. The paper describes how the semantic resource description models enable ExoGENI to autonomously instantiate on-demand virtual topologies of virtual machines provisioned from cloud providers and are linked by on-demand virtual connections acquired from multiple autonomous network providers to serve a variety of applications ranging from distributed system experiments to high-performance computing.

==> alg_path.tex <==

\noindent \textbf{Input:} $M_s$, $P(S,D,C)$

\noindent \textbf{Output:} $P_s=\{S_s,H_s^1,...,H_s^i,...,D_s\}$.

\begin{tabbing}
\= \ \ \ \ \ \ \= \ \ \ \ \= \ \ \ \ \= \ \ \ \ \= \ \ \ \ \=\kill
\>While(attempts++ $<$ limit)\\
\>\> Run Dijkstra Shortest Path Algorithm \\
\>\>\> Using {\it gleen:OnPath} to find the next hop\\
\>\>\>  {\it p} = the next shortest path between S and D\\
\>\>\> if {\it p=null}, return null \\
\>\> Validate path p \\
\>\>\> Using {\it gleen:subGraph} to get the list of \\
\>\>\>internal elements of {\it p} \\
\>\>\>\> Validate the label availability\\
\>\>\>\> Validate the bandwidth constraint \\
\>\>If {\it p} is valid, return $P_s(S,D,C)$ with internal \\
\>\>elements\\
\>\>else mark p unavailable and go back step 3\\
\>End while\\
\end {tabbing}


==> applying.tex <==

\subsection{NDL-OWL Models}

As described in Section~\ref{sec:using}, NDL-OWL defines multiple models for describing the various types of resource descriptions used by ORCA within ExoGENI, as shown in Table~\ref{tab:models}. Figure~\ref{fig:cycle} shows how the different models are exchanged between different actors. The models are generated dynamically and exchanged by various ORCA actors in the form of RDF-XML documents using an RPC interface, in a departure with the Linked Data approach common in the Semantic Web community. 

Users submit their requests to the ORCA controllers in the form of a request model that contains the {\em Reservation} instance which includes a variety of elements describing the needed resources, their topology, the term of the request and other configuration properties, like link bandwidth and OS images to be used on the compute resources. Requests may not be fully specified with respect to binding resources to specific domains, thus leaving it up to the controller to decide which specific provider sites the embedding should take place at.

Resource providers represented by ORCA Aggregate Managers (AMs) delegate abstractions of their resources using abstract delegation models to the ORCA Brokers. Controllers query brokers for these models in order to perform topology embedding. Brokers issue tickets for resources which permit controllers to instantiate the necessary resources at selected AMs and stitch them together. The controllers return the manifest model, which merges the information about instantiated resources with the original request model, to the user to enable the user access to the newly provisioned virtualized infrastructure of the slice.

%{\bf Substrate Description model:}
%This is the detailed resource and topology model that is used to describe a physical substrate including network topology and edge resources (compute and storage). ORCA AMs use this model to drive their internal resource allocation policies and resource configuration (setup/teardown handler invocations). The model also specifies which elements of the structure are exposed externally (e.g., in resource advertisements or delegations), and which are kept hidden. This feature provides the ability for providers to filter information exposed about their substrate, which is a common requirement of e.g. telecom network providers.
%
%{\bf Substrate Delegation model:}
%This is the abstract model to advertise an aggregate's resources and services externally. ORCA AMs use this representation to delegate advertised resources to ORCA broker(s). AMs may also use this representation to describe resources in response to queries. This mode allows multiple abstraction levels, as different AMs may want to expose different levels of resource and topology description of its substrate. 
%
%{\bf Slice Request model:} 
%This is the abstract model to represent user resource requests. A typical request might be a virtual topology with specific resources at the edges, generated by some experiment control tool. Our implementation allows the submission of a request via a GUI, automatic generation of a request from a point-and-click interface and the use of an XMLRPC API for submission and monitoring of the state of the request.

%The topology request can be {\em bound} or {\em unbound} depending on whether the endpoints of connections are required to end in specific domains or not. An unbound request can ask for a specific topology but not specify where it must be embedded. A bound request can ask to connect resources at several specific sites together. 
%Any request can also specify the amount of requested edge resource type (e.g. number of VMs). 
%For bound requests the controller can perform inter-domain path or topology computation based on the request and a description of the global topology collected from abstract delegated models, and automatically create sub-requests for each domain for allocation of network resources (e.g. circuits) or edge resources. For unbound requests the controller locates the sites with available resources to perform the topology embedding, thus binding the request to a specific site or sites. The controller also performs stitching of resources provisioned by multiple providers \cite{orca:mens10}.

\begin{figure}[t]\begin{center}  
\includegraphics[width=0.45\textwidth]{cycle}        
	\caption{NDL-OWL models in ORCA.}
	\label{fig:cycle}
\end{center}
\vspace{-0.3in}
\end{figure}

%\begin{figure}
%\label{fig:flukes}
%\centering
%\begin{minipage}{0.45\textwidth}
%\centering
%\includegraphics[width=\textwidth]{cycle}
%\caption{NDL-OWL models in ORCA.}
%\end{minipage}
%\begin{minipage}{0.45\textwidth}
%\centering
%\includegraphics[width=\textwidth]{flukes}
%\caption{Flukes screenshot showing the requested slice topology (upper left) and slice manifest (lower right).}
%\end{minipage}
%\end{figure}
%
%\begin{figure}[t]\begin{center}  
%\includegraphics[width=0.5\textwidth]{cycle}        
%	\caption{NDL-OWL models in ORCA. }
%	\label{fig:cycle}
%\end{center}
%\end{figure}

%{\bf Slice Reservation model:}
%This is the abstract model used by ORCA brokers to return resource tickets to the controller. Each ticket contains information on one or more slivers allocated from a specific AM named in the ticket. The controller obtains the slivers by redeeming these tickets to the AMs. This model describes the interdependency relationships among the slivers so that the SM controller can drive stitching information for each sliver into the slice. Currently, ORCA uses the substrate delegation model: the ticket contains a resource type and unit count for the resources promised in the ticket, together with the complete original advertisement from the AM.
%
%{\bf Slice Manifest model:}
%This is the abstract model to describe the topology, access method, state, and other post-configuration information of the slice {\em as built}. It contains detailed information about instantiated resources and access methods for tools or users to interact with them.

%Figure 3 shows the paths along which the various models are exchanged between various ORCA actors.

%\vspace{-0.1in}
%\subsection{Semantic tools in ExoGENI}
%
%ORCA relies on Jena framework~\cite{JENA} for operating on NDL-OWL models. In addition to using the semantic resource representations internally, we have developed a number of tools that leverage JENA and NDL-OWL for various purposes. 
%
%One of these tools is called {\em Flukes}. It is a GUI built for assisting users in creating slice request models and visualizing the manifest models. A screenshot of Flukes is shown in Figure 4. The request model includes several clusters bound to different cloud providers. Since the cloud providers are not directly connected to each other, ORCA acquired and stitched together the necessary intermediate links which are shown in the manifest view. 

%\begin{figure}[h]
%  \begin{center}
%    \includegraphics[width=0.60\textwidth]{flukes.pdf}
%  \end{center}
%  \caption{Flukes screenshot showing the requested slice topology (upper left) and slice manifest (lower right).}
%  \label{fig:flukes}
%\end{figure}

%ExoGENI is unique within GENI in relying on semantic resource description mechanisms. The other frameworks in the GENI federation rely on traditional XML-schema based representations, referred to as {\em RSpecs}~\cite{rspec}. In order to interoperate with the rest of GENI it became necessary to create a translation service between RSpecs and NDL-OWL. NDL-OWL models are more expressive than RSpecs, so the translation service generally provides the subset information contained in the NDL-OWL representations - the minimal amount necessary for supporting inter-operability. This conversion service also leverages JENA as well as standard Java XML parsing tools like Xerces and JAXB to perform the conversions. The following conversion functions are currently available:
%
%\begin{itemize}
%\item Conversion from RSpec requests to NDL-OWL requests to enable GENI tools based on RSpecs to request resources from ExoGENI and ORCA.
%\item Conversion from NDL-OWL manifests to RSpec manifests. 
%\item Conversion from NDL-OWL abstract substrate descriptions to RSpec {\em advertizements}.
%\end{itemize}
%
%The conversion service is hosted in a number of locations as an XMLRPC web-service with self-documented calls by using XMLRPC introspection\footnote{http://geni.renci.org:12080/ndl-conversion/convert.jsp}.

%\subsection{Stitching}
%
%A critical challenge in distributed cloud orchestration is stitching of slivers that cross domain boundaries.  A key example is stitching links across multiple network aggregates. A cross-aggregate network stitch involves a link that crosses a border between two adjacent providers. The border link connects a switch owned by one provider to a switch owned by the other. The network stitching problem is also faced by inter-domain circuit services~\cite{dragon07}.
%
%% We focus on the mechanics of stitching the slivers to create an end-to-end virtual
%% topology, given a suitable mapping of slivers to aggregates.
%
%
%In general, instances of stitching that are currently understood involve linking two slivers that are adjacent at a common underlying substrate component.  One sliver is named by a label that is installed in the other.  For example, to stitch a VM to a VLAN with a given tag, we instantiate a virtual network interface bound to the VLAN tag within the VM.  The virtual interface is instantiated from a physical network interface in the underlying host that runs the VM.  The physical interface must be adjacent to a switch port that exposes a VLAN named by the specified tag.  The aggregate that hosts the VLAN sliver produces the tag.  The aggregate that hosts the VM sliver consumes the tag.
%
%The producer and consumer of the tag might or might not be the same aggregate.  Stitching across aggregates---or across slices---requires suitable authorization.  In particular, some coordinator must act as a common trust anchor to endorse the parties to one another, unless they have direct knowledge of the relevant public keys (e.g., aggregate operators may install keys for aggregates that are adjacent in the network).
%
%Some legacy network components cannot accept an arbitrary label value chosen by a producer.   For these types it is necessary to negotiate a value that is acceptable to both slivers involved in the stitch, and/or their hosting components.  The label value constraints may propagate transitively if multiple slivers are chained together, and they are hosted on components lacking a translation capability.  Such limitations complicate the stitching architecture.
%
%ORCA provides a general facility for cross-aggregate stitching that applies for network stitching and other stitching use cases as well.  This feature enables ORCA to orchestrate end-to-end stitching across multiple aggregates. It can incorporate inter-domain circuit services offered by third parties, as outlined above, but where ``air gaps'' exist between circuit services ORCA may bridge
%them by cross-aggregate stitching at exchange points.
%
%For example, as discussed in Section~\ref{sec:exchange}, ExoGENI has an exchange aggregate at the StarLight exchange facility. The AM controls a single node (a switch), whose interfaces are connected to links to switches owned by other transport networks with a presence at StarLight, including NLR, Internet2, and ESNet/ANI. The switch is an Ethernet switch (a Cisco 6509) with a {\it swapping} capability, also called VLAN tag remapping or VLAN translation. To join two pipes to form a circuit spanning StarLight, two adjacent networks produce VLAN tags for the circuit on their adjacent links.   The AM joins them by consuming the selected VLAN tags and remapping them at each interface (port) to the same internal tag. 
%
%All sliver stitching in ORCA follows this producer/consumer model.  Creating a stitch is a two-step process.  First, the controller allocates a sliver from the producer, which selects a tag or label for it, perhaps guided by a broker or other coordinator. The label is chosen from some namespace associated with the adaptation, such as the set of legal VLAN tags.   Second, the controller passes the label securely in a request to join the labeled sliver to another adjacent sliver (the consumer). The controller queries the domain models of the aggregates hosting those slivers to infer which is the producer and which is the consumer, based on their capabilities (e.g., swapping). In this way, the controller constructs a directed dependency DAG as it plans a slice's virtual topology and the mapping to aggregates. The nodes of the DAG are slivers, and the DAG has directed edges from producers to consumers. The controller then traverses the DAG, instantiating slivers and propagating labels to their successors as the labels become available.
%
%The BEN circuit service also has a swapping capability. At present, many of the external circuit services do not, but we hope and expect that they will add it in the near future. When two providers are adjacent at a link and neither has swapping capability, various standards and approaches exist to negotiate common tags.  

